Inverse Optimal Control Design of a VTOL Aircraft

A Vertical Takeoff and Landing (VTOL) aircraft is capable of short/vertical takeoffs and landings, thus eliminating the requirement of long runways. This feature makes them suitable for a broader variety of missions, generally not achievable by a traditional aircraft. The dynamics of the VTOL aircraft in the vertical plane has been used as a benchmark problem to demonstrate the effectiveness of different nonlinear control techniques, mainly due to being highly coupled and non-minimum phase. This paper presents the design of an inverse optimal control for a simplified VTOL aircraft model. The proposed control law is based on a Control Lyapunov Function (CLF) which exploits the normal form typically used for control design through feedback linearization. The suggested control law is compared with dynamic feedback linearization based control law and a comparison is drawn based on their efficacy and robustness.

==> FiguresTikz.tex <==
\begin{tikzpicture}[/tikzinclude/figure=BlkDiag,BlockDiagram,node distance = 2cm,>=latex']
\node[block,blue!75!black,   fill=blue!20]   at ( 1.75,0) (P1) {\Large$\Sigma$};
\node[block,red!75!black, fill=red!20] at ( 0.0,0) (S1) {\Large$\delta$};
\node[block,blue!75!black,   fill=blue!20]   at (-1.75,0) (P2) {$k(x)$};

\draw[->,thick] (P1) -| +(1,-1) node[above,pos=0.25] {$x$} -- +(-4.5,-1)|- (P2);
\draw[->,thick] (S1) -- (P1) node[above,pos=0.5] {$u$};
\draw[->,thick] (P2) -- (S1);
\end{tikzpicture}


\begin{tikzpicture}[/tikzinclude/figure=PVTOL,BlockDiagram,node distance = 2cm,>=latex']
\begin{scope}[rotate=20]
	\draw[->] (2,-0.3) -- (1,-2.15);
	\draw[dashed] (2,-0.3) -- (0,-4);
	\draw[->] (-2,-0.3) -- (-1,-2.15);
	\draw[dashed] (-2,-0.3) -- (0,-4);
	\draw[->] (0,0) -- (0,-2);
	\draw[dashed] (0,0) -- (0,-4);
	\draw[thick,blue!75!black,fill=blue!20] (0,1.5) -- (0.1,0.4) -- (3.5,-0.5) -- (3.0,-0.6) -- (0.5,-0.3) -- (0.2,-0.9) -- (-0.2,-0.9) -- (-0.5,-0.3) -- (-3.0,-0.6) -- (-3.5,-0.5) -- (-0.1,0.4) -- cycle;
	
	\draw[-] (0,0) -- +(0,2.5);
	\draw[-] (0,0) -- +(0.8551,2.3492);
	\draw[<-] (0,2.3) arc (90:70:2.3) node[above,pos=0.5] {$\theta$};
	
	\draw[dashed] (0,0) -- +(2.5,0);
	\draw[dashed] (0,-4) -- +(2.5,0);
	\draw[<->] (2.2,0) -- +(0,-4) node[right,pos=0.5] {$r$};
	
	\draw[->, very thick] (0,-4) -- +(1.5,0) node[below right,pos=0.8] {$F_1$};
	\draw[->, very thick] (0,-4) -- +(0,1.5) node[above right,pos=0.8] {$F_2$};
\end{scope}
\begin{scope}[scale=0.2,rotate=20]
	\draw[fill=black] (0,0) -- (1,0) arc (0:90:1) -- (0,0);
	\draw[fill=black] (0,0) -- (-1,0) arc (180:270:1) -- (0,0);
	\draw[fill=white] (0,0) -- (0,1) arc (90:180:1) -- (0,0);
	\draw[fill=white] (0,0) -- (0,-1) arc (270:360:1) -- (0,0);
	\draw[black] (0,0) circle (1);
\end{scope}
\draw[->, very thick] (-2,-4) -- +(1.5,0) node[below right,pos=0.8] {$x$};
\draw[->, very thick] (-2,-4) -- +(0,1.5) node[above right,pos=0.8] {$y$};
\end{tikzpicture}


